Understanding and Mitigating the Threat of Vec2Text to Dense Retrieval Systems

The emergence of Vec2Text -- a method for text embedding inversion -- has raised serious privacy concerns for dense retrieval systems which use text embeddings, such as those offered by OpenAI and Cohere. This threat comes from the ability for a malicious attacker with access to embeddings to reconstruct the original text. In this paper, we investigate various factors related to embedding models that may impact text recoverability via Vec2Text. We explore factors such as distance metrics, pooling functions, bottleneck pre-training, training with noise addition, embedding quantization, and embedding dimensions, which were not considered in the original Vec2Text paper. Through a comprehensive analysis of these factors, our objective is to gain a deeper understanding of the key elements that affect the trade-offs between the text recoverability and retrieval effectiveness of dense retrieval systems, offering insights for practitioners designing privacy-aware dense retrieval systems. We also propose a simple embedding transformation fix that guarantees equal ranking effectiveness while mitigating the recoverability risk. Overall, this study reveals that Vec2Text could pose a threat to current dense retrieval systems, but there are some effective methods to patch such systems.

==> sections/corpus_poison.tex <==
\begin{table*}[!htp]\centering
\captionsetup{skip=5pt}
	\caption{Results of applying Vec2Text to the task of corpus poisoning, compared to existing HotFlip approach. Vec2Text has the advantage of being able to produce numerous adversarial passages ($k$) without model weights. Both Vec2Text and HotFlip are well below the upper bound, indicating that better methods could pose a serious risk in corpus poisoning.}\label{tab:poision}
		\begin{tabular}{@{}lrrrrr@{}}\toprule
			\bf Attack method & \bf \#Adversarial Passages / & \bf Success@10 & \bf Success@20 & \bf Success@100 & \bf Success@1000 \\
%			& \bf  / \\
			& \bf Query Clusters $k$ \\
			\midrule
			HotFlip~\cite{zhong-etal-2023-poisoning} &10 &0.006 &0.015 &0.105 &0.532 \\
			Vec2Text & 10 &0.006 &0.012 &0.036 &0.101 \\
			\hspace{5pt} Query centroid (upper bound) &10 &0.206 &0.304 &0.575 &0.926 \\
			\hline
			HotFlip & 100 & $\cdots$ & \multicolumn{3}{c}{\small Too computationally expensive} $\cdots$  \\
			Vec2Text &100 &0.061 &0.091 &0.189 &0.401 \\
			\hspace{5pt} Query centroid (upper bound) &100 &0.493 &0.620 &0.868 &0.994 \\
			\hline
			HotFlip & 1000 & $\cdots$ & \multicolumn{3}{c}{\small Too computationally expensive} $\cdots$  \\
			Vec2Text &1000 &0.268 &0.335 &0.521 &0.791 \\
			\hspace{5pt} Query centroid (upper bound) &1000 &0.779 &0.873 &0.980 &1.000 \\
			\bottomrule
		\end{tabular}
\end{table*}


\section{A New Threat: Corpus Poisoning}
In this section, we investigate whether Vec2Text poses a threat to existing DR systems through a corpus poisoning attack.

\subsection{Existing Corpus Poisoning Attack Method}
A corpus poisoning is an adversarial attack where a malicious user injects adversarial passages into a retrieval corpus with the intention of misleading DR models. This is a relatively new type of attack, and, to date, there is only one existing study conducted on this problem~\cite{zhong-etal-2023-poisoning}. Specifically, \citet{zhong-etal-2023-poisoning} proposed a gradient-based approach, inspired by the HotFlip method~\cite{ebrahimi-etal-2018-hotflip,wallace-etal-2019-universal}, which generates a small set of adversarial passages by perturbing discrete tokens in randomly initialized passages to maximize their similarity with a provided set of training queries. These adversarial passages are then inserted into the retrieval corpus, and the success of the attack is determined by the retrieval of these adversarial passages at a high rank in response to future unseen queries. These adversarial passages can be used to harm retrieval effectiveness and/or inject spam or content with misinformation into the search engine result list.

The current HotFlip-based corpus poisoning method has two drawbacks (that is, from an attacker perspective). Firstly, being a gradient-based method, it requires access to the embedding model weights, i.e., it is a white box attack. Consequently, attackers cannot employ this method to target DR systems built with closed-source embedding models, such as OpenAI embedding models. Secondly, the method is iterative, with only one token in the adversarial passage selected and perturbed at each iteration. This process cannot be parallelized within each adversarial passage, as the perturbation of the next token depends on the previously perturbed token. 
This makes the method time-consuming and resource intensive: in our experiments with a single H100 GPU, HotFlip takes approximately 2 hours to generate a single adversarial passage. 

\subsection{Performing Corpus Poisoning with Vec2Text}

In contrast, Vec2Text does not suffer from the drawbacks of HotFlip. 
First, Vect2Text does not require access to the embedding model weights. Once Vec2Text is trained, it can directly generate the adversarial passage from the embedding using standard language model generation inference. Second, it allows for efficient generation of a large set of adversarial passages (being far less computationally intensive than HotFlip).

To formally define corpus poisoning with Vec2Text, let $\mathcal{Q}=\{q_1, q_2, ..., q_{|\mathcal{Q}|}\}$ be a set of training queries. The goal is to use Vec2Text to generate an adversarial passage $a$ whose embedding maximizes the similarity to all the training query embeddings:
\begin{align}
	a &= \underset{a'}{\mathrm{argmax}} \frac{1}{\mathcal{|Q|}} \sum_{q_i \in \mathcal{Q}} \phi(q_i)^\transp \phi(a') \\
	&=\underset{a'}{\mathrm{argmax}} \: \phi(a')^\transp \frac{1}{\mathcal{|Q|}} \sum_{q_i \in \mathcal{Q}} \phi(q_i) \\
	&=\underset{a'}{\mathrm{argmax}} \: \phi(a')^\transp \phi_{\mathcal{Q}},
\end{align}
where $\phi_{\mathcal{Q}}$ is the average embedding or centroid embedding of all the training query embeddings. The maximum similarity is achieved when $\phi(a') = \phi_{\mathcal{Q}}$. Vec2Text can solve this optimization problem through a three-stage process:
\begin{itemize}
	\item The first stage is the standard training of Vec2Text (i.e., reconstructing the text for any given embedding). 
	\item The second stage involves computing the centroid embedding $\phi_{\mathcal{Q}}$ of training queries, which can be done by sending the training queries to the embedding model to obtain all the query embeddings and averaging them. 
	\item Finally, inputting $\phi_{\mathcal{Q}}$ to the trained Vec2Text yields a generated text, which is the adversarial passage $a$.
\end{itemize}  
A perfect Vec2Text would generate an adversarial passage whose embedding is exactly the same as the query centroid; i.e., $\phi(a) = \phi_{\mathcal{Q}}$. 

Once again, we emphasize that the entire process does not require access to model weights. Moreover, generating an adversarial passage with Vec2Text is efficient: 
generating a single passage took 5 seconds on a single H100 GPU, employing beam search with 50 steps and a width of 4.



\subsection{Corpus Poisoning Experiments}

\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
		$a$ = {\ttfamily "That drawings promises Key kot iner jor Respond machines AK <pad> ance pe izi very nie <pad> <pad> Doar ceapa Weg MEN Am OK Jamie words Um Imp refers '' War Hop nism the serving Bol auto Palatul fries rome lighter (1 49 fetch 19 cities can counting 16, As"}
        \caption{HotFlip. Cosine similarity of this passage to the query centroid embedding is $\cos(\phi(a), \phi_{\mathcal{Q}}) = 0.96$.}
    \end{subfigure}
    \\[1em]
    \begin{subfigure}{0.45\textwidth}
	$a$ = {\ttfamily "when does the 7 episode season of the new two come out </s>"}
        \caption{Vect2Text. Cosine similarity of this passage to the query centroid embedding is $\cos(\phi(a), \phi_{\mathcal{Q}}) = 0.85$.}
    \end{subfigure}
\caption{Sample adversarial passages most closely matching the NQ training query centroid.}
    \label{fig:passage}
\end{figure}


We conducted the corpus poisoning experiments with the GTR-base embedding model (with correct embeddings) as the target DR system, utilizing the NQ datasets as the target corpus. 
NQ training queries are used to first encode the query centroid embedding and then to generate adversarial passages. In practice, we generate multiple adversarial passages (in line with \citet{zhong-etal-2023-poisoning}). This was done by first using $k$-means clustering to cluster the training queries based on their embeddings. Once the queries are grouped into clusters, we take the centroid embedding of each cluster and input them to Vec2Text to generate one adversarial passage for each cluster. We set $k$ to $10, 100, 1000$.

Evaluation was then done using NQ test queries. The evaluation measure is $Success@n$ (in line with~\cite{zhong-etal-2023-poisoning}), which represents the percentage of queries for which at least one adversarial passage is retrieved in the top-$n$ results. A higher success rate indicates a greater vulnerability to corpus poisoning. 

Table~\ref{tab:poision} presents corpus poisoning results. When only 10 adversarial passages are generated (grouping training queries with 10-means clustering), both HotFlip and Vec2Text perform poorly on success@10 and 20; however, HotFlip does work when injecting adversarial passages into the top 100 or 1000 rank positions. If the embedding model weights are available, HotFlip is a more potent corpus poisoning attack method when applied to longer rank lists of 100 or 100.

Vec2Text has the advantage of being able to generate many more adversarial passages; when $k=100$ or $k=1000$ HotFlip is too computationally expensive and thus largely impractical. For these cases Vec2Text success rate improves, with $k=1000$ making Vec2Text a considerable threat in corpus poisoning. 

The adversarial passages are generated from query embeddings and are such synthetic and may not appear like real passages. Figure~\ref{fig:passage} shows the two adversarial passages most closely matching a sampled query centroid $\phi_{\mathcal{Q}}$ for both HotFlip and Vec2Text. The cosine similarity with the query centroid embeddings is also reported in the caption. Recall that HotFlip works by flipping tokens one at a time, whereas Vec2Text is a language model decoder. This difference may explain by Vec2Text appears to generate more natural language. 

The embeddings of the adversarial passages in Figure~\ref{fig:passage} still differ from the query centroid embeddings (cosine similarity being 0.96 for HotFlip and 0.85 for Vec2Text). Recall that a perfect Vec2Text would generate an adversarial passage for which the embedding is exactly the same as the query embedding. To understand how this best case scenario affects success@k we run an additional experiment which involved directly inserting the query centroid embeddings into the vector index and then evaluating the success@k. This serves as an upper bound for the HotFlip and Vec2Text corpus poisoning attacks --- an analysis overlooked in the original corpus poisoning paper~\cite{zhong-etal-2023-poisoning}. Results are shown in Table~\ref{tab:poision} as "Query centroid (upper bound)". For both different values of $k$ and different success@$n$, the upper bound is much higher than both HotFlip or Vec2Text. This tells us that neither method is optimal yet for the corpus poisoning attack. It also highlights that if a much more effective corpus poising method --- one closer to the upper bound --- was developed, it could have serious adverse consequences for dense retrievers.





  






==> sections/results.tex <==
\section{Results and Analysis}


\subsection{Reproducing with the correct GTR embedding}

\begin{table*}[!htp]\centering
	\caption{Reproduced results.}\label{tab: reproduce}
	\resizebox{0.9\textwidth}{!}{
	\begin{tabular}{l|llll | llll}\toprule
		\multirow{2}{*}{Embedding Models}&\multicolumn{4}{c|}{Retrieval effectiveness} & \multicolumn{4}{c}{Reconstructability} \\\cmidrule{2-9}
		 &top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
		gtr-base (original) &0.634 &0.711 &0.816 &0.893 &90.128 &0.970 &0.758 &0.990 \\
		gtr-base (reproduced) &0.634 &0.711 &0.816 &0.893 &88.956 &0.971 &0.699 &0.996 \\
		gtr-base-st (bug fixed) &0.718 &0.773 &0.855 &0.913 &90.362 &0.970 &0.752 &0.998 \\ \hline
		DPR\_cls &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
		DPR\_cos &0.748 &0.799 &0.863 &0.914 &71.834 &0.879 &0.345 &0.975 \\
		DPR\_mean\_cos &0.745 &0.802 &0.866 &0.916 &81.918 &0.924 &0.480 &0.988 \\\hline
		BERT\_cls & 0.101 & 0.153& 0.288 &0.467 & 37.034& 0.671& 0.042& 0.968 \\
		BERT\_mean\_cos &  0.283& 0.358& 0.520 & 0.715 & 80.057&0.914 &0.414 & 0.984\\\hline
		SimLM-cls & 0.304  & 0.378& 0.546 & 0.720 & 94.560& 0.974& 0.677& 0.999 \\
		SimLM-cls-finetuned & 0.750 & 0.805& 0.874 & 0.919 & & & & \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Impact of distance metric and pooling}

\subsection{Impact of adding noise to the embedding}

\begin{table*}[!htp]\centering
	\caption{Impact of adding noise to the embedding}\label{tab:noise}
	\scriptsize
		\resizebox{1\textwidth}{!}{
	\begin{tabular}{l|llll|llll|llll}\toprule
		\multirow{2}{*}{Embedding Models}&\multicolumn{4}{c|}{Retrieval effectiveness} &\multicolumn{4}{c|}{Reconstruct effectiveness} &\multicolumn{4}{c}{Noise Reconstruct effectiveness} \\\cmidrule{2-13}
		&top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos &bleu &tf1 &exact &cos \\\midrule
		DPR\_cls &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 &10.022 &0.415 &0.000 &0.823 \\
		DPR\_cls\_noise &0.730 &0.790 &0.856 &0.911 &29.264 &0.635 &0.012 &0.966 &17.417 &0.504 &0.005 &0.882 \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Impact of embedding dimension and quantization}
\begin{table*}[!htp]\centering
	\caption{Impact of embedding dimension and quantization.}\label{tab: dim}
	\scriptsize
			\resizebox{1\textwidth}{!}{
	\begin{tabular}{l|l|llll|llll}\toprule
		\multirow{2}{*}{Embedding Models}&Index size &\multicolumn{4}{c|}{Retrieval effectiveness} &\multicolumn{4}{c}{Reconstruct effectiveness} \\\cmidrule{2-10}
		&GB &top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
		DPR\_cls\_768 &61G &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
		DPR\_cls\_256 &21G &0.731 &0.784 &0.855 &0.910 &25.060 &0.565 &0.035 &0.881 \\
		DPR\_cls\_PQ\_m768 &16G &0.749 &0.801 &0.862 &0.914 &1.916 &0.146 &0.000 &0.748 \\
		DPR\_cls\_PQ\_m256 &5.3G &0.740 &0.796 &0.864 &0.912 &2.305 &0.159 &0.000 &0.767 \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Customized embedding transformation}

\begin{table*}[!htp]\centering
	\caption{Impact of customized embedding transformation.}\label{tab:tranformation}
	\scriptsize
				\resizebox{0.9\textwidth}{!}{
	\begin{tabular}{l|llll|llll}\toprule
		\multirow{2}{*}{Embedding Models}&\multicolumn{4}{c}{Retrieval effectiveness} &\multicolumn{4}{c}{Reconstruct effectiveness} \\\cmidrule{2-9}
		&top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
		DPR\_cls &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
		DPR\_cls\_transform &0.748 &0.800 &0.863 &0.914 &1.178 &0.065 &0.000 &0.443 \\
		\bottomrule
	\end{tabular}
}
\end{table*}


\subsection{Apply vec2text to corpus poisoning attack}

\begin{table*}[!htp]\centering
	\caption{Corpus poisoning results.}\label{tab:poision}
	\scriptsize
	\resizebox{0.9\textwidth}{!}{
		\begin{tabular}{l|l|llll}\toprule
			Attack method &\#  adv. pass. &Recall@10 &Recall@20 &Recall@100 &Recall@1000 \\\midrule
			hotflip &10 &0.006 &0.015 &0.105 &0.532 \\
			vec2text &10 &0.006 &0.012 &0.036 &0.101 \\
			Oracle &10 &0.206 &0.304 &0.575 &0.926 \\\hline
			vec2text &100 &0.061 &0.091 &0.189 &0.401 \\
			Oracle &100 &0.493 &0.620 &0.868 &0.994 \\\hline
			vec2text &1000 &0.268 &0.335 &0.521 &0.791 \\
			Oracle &1000 &0.779 &0.873 &0.980 &1.000 \\
			\bottomrule
		\end{tabular}
	}
\end{table*}



